Continual Depth-limited Responses for Computing Counter-strategies in Sequential Games

In zero-sum games, the optimal strategy is well-defined by the Nash equilibrium. However, it is overly conservative when playing against suboptimal opponents and it can not exploit their weaknesses. Limited look-ahead game solving in imperfect-information games allows defeating human experts in massive real-world games such as Poker, Liar's Dice, and Scotland Yard. However, since they approximate Nash equilibrium, they tend to only win slightly against weak opponents. We propose methods combining limited look-ahead solving with an opponent model in order to 1) approximate a best response in large games or 2) compute a robust response with control over the robustness of the response. Both methods can compute the response in real time to previously unseen strategies. We present theoretical guarantees of our methods. We show that existing robust response methods do not work combined with limited look-ahead solving of the shelf, and we propose a novel solution for the issue. Our algorithm performs significantly better than multiple baselines in smaller games and outperforms state-of-the-art methods against SlumBot.

==> old_sections/01_introduction.tex <==
\section{Introduction}

Researchers aim to solve bigger and bigger games. A breakthrough that allowed defeating human experts in several large imperfect-information games is limited look-ahead solving, which adapts a well-known approach from perfect-information games to games with imperfect-information \cite{moravvcik2017deepstack, brown2019superhuman, schmid2021player}. Limited look-ahead solving takes advantage of decomposition. It builds the game to some depth and solves it using a value function that can be learned, for example, by neural networks. When the depth-limit is reached, we build another part until the depth-limit and continue until the end of the game.

All the existing algorithms of this type assume perfect rationality of the opponent and do not allow explicit modeling of an opponent and exploitation of his mistakes. As a result, even very weak opponents exploitable by the heuristic local best response (LBR) \cite{lisy2017eqilibrium} can tie or lose very slowly against these methods \cite{zarick2020unlocking}. As more and more computer-generated strategies are deployed in the real world \cite{an2013deployed} we can not avoid the interaction of AI systems with humans. Therefore, there has been a significant amount of work towards computing strategies to use against imperfect opponents such as humans \cite{bard2013online, wu2021l2e, southey2012bayes, mealing2015opponent, korb2013bayesian, milec2021complexity, johanson2009data}. We continue this area of research and propose the first algorithms that allow opponent modeling in limited look-ahead solving in imperfect-information games.

First, we propose a continual depth-limited best response (CDBR), which fixes the opponent and does continual resolving. Assuming we had precise value function\footnote{the Value function takes player's reaches at the depth limit and returns the evaluation of the information sets for both players.} trained to return values as if we played against a particular opponent, and the algorithm would produce the best response (BR). Next, we propose continual depth-limited restricted Nash response (CDRNR), which is based on restricted Nash response (RNR) \cite{johanson2008computing} with modifications to allow depth-limited solving. Specifically, we need to measure the increase in exploitability caused by the change in our strategy, which is done by computing BR in RNR. To do that precisely, we keep all the previously considered parts of the game and show the problems caused by replacing them with known gadgets \cite{burch2014solving,moravcik2016refining,brown2017safe}.

To avoid training a vast amount of value functions, we use the single (optimal) value function, which assumes both players act rationally after the depth limit. As a result, we create algorithms that do not directly compute BR and RNR but still have favorable theoretical guarantees and practical results. We propose first algorithms that allow real-time opponent modeling in large extensive-form games (EFGs). Specifically, CDBR is a generalization of LBR. Compared to previous approaches using reinforcement-learning \cite{heinrich2016deep, mnih2013playing,timbers2020approximate}, we can quickly compute the response to an unseen opponent model. Therefore, it is the first algorithm approximating BR in large games applicable in real-time opponent modeling. CDRNR has no comparison since no other algorithm is trying to compute robust responses in large EFGs, making it the first robust response that can be quickly recomputed for unseen opponent models.

Authors in \cite{liu2022safe} propose similar approach called Safe Exploitation Search (SES) but the algorithm often fails to exploit the opponent. We show a counterexample to the main Theorem they formulate about the bounded exploitability based on our gadget analysis. It nicely illustrates the complexity of the problem and that the issues are not easily identifiable. We also compare with their approach experimentally.

Our contributions are: \textbf{1)}  We formulate the algorithms to find the responses given opponent strategy and an evaluation function, resulting in the first robust response applicable to massive games. \textbf{2)} We prove the soundness of the proposed algorithms. \textbf{3)} We empirically evaluate the algorithms on three different games and compare it to SES. We show that our responses exploit the opponents, and CDBR outperforms domain-specific local best response \cite{lisy2017eqilibrium} on poker.

% Limited look-ahead game solving for imperfect information games is the breakthrough that allowed defeating expert humans in several large games. 

% A breakthrough in solving massive imperfect-information EFGs was the depth-limited solving, which builds the game until a depth limit and evaluates the rest using a value function\footnote{Value function takes player reaches at the depth limit and returns the evaluation of the information sets for both players.} \cite{moravvcik2017deepstack, brown2018superhuman, schmid2021player}. It allowed defeating expert humans in several large games. However, the existing algorithms of this type assume the perfect rationality of all the players and do not allow modeling and exploitation of the opponent's flaws.

% More and more computer-generated strategies are deployed in the real world \cite{an2013deployed, fang2017paws}, and we can not avoid the interaction of AI systems with humans. This interaction might be cooperative, but in many cases, for example, in both network security and physical security, it is usually competitive. Therefore, there has been a significant amount of work towards computing strategies to use against imperfect opponents such as humans \cite{bard2013online, wu2021l2e, southey2012bayes, mealing2015opponent, korb2013bayesian, milec2021complexity, johanson2009data}. We focus on extensive-form games (EFGs), a powerful model able to describe recreational games, such as poker, as well as real-world situations from physical or network security. In EFGs, many exploitative approaches use the best response or robust response, either to respond to an explicit model of the opponent or to create a portfolio of exploitative strategies beforehand \cite{bard2013online, ganzfried2011game}. Moreover, evaluating equilibrium strategies through exploitability is common in the literature, and we need to compute best responses to do that.

% However, real-world games are often massive, and in such games, computing the best response or robust response is intractable. There are approaches to approximate best response using frequentist best response with abstraction \cite{johanson2008computing} or by learning the response using deep reinforcement learning \cite{heinrich2016deep, mnih2013playing}. Nevertheless, none of those approaches have theoretical guarantees, and the responses using deep reinforcement learning can not be quickly applied to various opponent models without costly re-training \cite{timbers2020approximate}. We want to guarantee that the response will achieve at least the value of the game against the strategy we are responding to. Furthermore, we want the robust response to have a guaranteed upper bound on the exploitability of the resulting strategy. This ensures that we will always be gaining against the model, and what we lose when the model is incorrect will be bounded. We want to have a response that can be quickly computed against different models, and we only allow precomputed statistics for the game, not for a specific opponent model.

% A breakthrough in solving massive imperfect-information EFGs was the depth-limited solving, which builds the game until a depth limit and evaluates the rest using a value function\footnote{Value function takes player reaches at the depth limit and returns the evaluation of the information sets for both players.} \cite{moravvcik2017deepstack, brown2018superhuman, schmid2021player}. We use depth-limited solving with a fixed opponent strategy to compute the responses. Unlike full best response which can be computed in one pass through the game tree, the depth-limited best response requires using an iterative CFR algorithm. Full best response can exploit opponent's weakness anywhere in her strategy, while using the optimal value function at a depth-limit prevents it.
% On the other hand, using the optimal value function independent of a specific opponent allows fast approximation of exploitability of any strategy \cite{lisy2017eqilibrium, timbers2020approximate}.

% Apart from best response, we focus on the restricted Nash response \cite{johanson2008computing}. It seeks a counterstrategy against an anticipated opponent's strategy, which is robust against any deviations from the anticipation. To guarantee the robustness of the response, we need an upper bound on exploitability even in the depth-limited scheme. Resolving gadgets \cite{burch2014solving, moravcik2016refining, brown2017safe} are tools used to guarantee no increase in exploitability in continual depth-limited solving. However, when we have a setup where we need to measure the change in exploitability in the gadget compared to what we can gain somewhere else in the game, the existing gadgets can provide wrong values. We explain and illustrate the problem and propose a novel gadget modification that solves the issue.

% Our contributions are: \textbf{1)}  We formulate the algorithms to find the responses given opponent strategy and an evaluation function, resulting in the first robust response applicable to massive games. \textbf{2)} We show a problem with gadget values and propose a new gadget to solve the problem. \textbf{3)} We prove the soundness of the proposed algorithms. \textbf{4)} We empirically evaluate the algorithms on three different games. We show that our responses exploit the opponents, and depth-limited best response outperforms domain-specific local best response \cite{lisy2017eqilibrium} on poker.

==> old_sections/02_background.tex <==
\section{Background}
\label{sec:background}
A two-player extensive-form game (EFG) consist of a set of players $N = \{\pr,\ps,c\}$, where $c$ denotes the chance, $\pr$ is the maximizer and $\ps$ is the minimizer. $A$ is a finite set of all actions available in the game. $H \subset \{a_1 a_2 \cdots a_n \mid a_j \in A, n \in \mathbb{N}\}$ is the set of histories in the game. We assume that $H$ forms a non-empty finite prefix tree. We use $g \sqsubset h$ to denote that $h$ extends $g$. The \textit{root} of $H$ is the empty sequence $\emptyset$. The set of leaves of $H$ is denoted $Z$, and its elements $z$ are called \textit{terminal histories}. The histories not in Z are \textit{non-terminal histories}. By $A(h) = \{a \in A \mid ha \in H\}$ we denote the set of actions available at $h$. $P : H \setminus Z \to N$ is the \textit{player function} which returns who acts in a given history. Denoting $H_i = \{h \in H\setminus Z \mid P(h) = i\}$, we partition the histories as $H = H_\pr \cup H_\ps \cup H_c \cup Z$. $\sigma_c$ is the \textit{chance strategy} defined on $H_c$. For each $h \in H_c, \sigma_c(h)$ is a fixed probability distribution over $A(h)$. Utility functions assign each player utility for each leaf node, $u_i : Z \to \mathbb{R}$. The game is of \textit{imperfect information} if some actions or chance events are not fully observed by all players. The information structure is described by \textit{information sets} for each player $i$, which form a partition $\Iset_i$ of $H_i$. For any information set $I_i \in \Iset_i$, any two histories $h, h' \in I_i$ are indistinguishable to player $i$. Therefore $A(h) = A(h')$ whenever $h, h' \in I_i$. For $I_i \in \Iset_i$ we denote by $A(I_i)$ the set $A(h)$ and by $P(I_i)$ the player $P(h)$ for any $h \in I_i$.

A \textit{strategy} $\sigma_i \in \Sigma_i$ of player $i$ is a function that assigns a distribution over $A(I_i)$ to each $I_i \in \Iset_i$. A \textit{strategy profile} $\sigma = (\sigma_\pr, \sigma_\ps)$ consists of strategies for both players. $\pi^\sigma(h)$ is the probability of reaching $h$ if all players play according to $\sigma$. We can decompose $\pi^\sigma(h) = \prod_{i \in N}\pi^\sigma_i(h)$ into each player's contribution. Let $\pi^\sigma_{-i}$ be the product of all players' contributions except that of player $i$ (including chance). For $I_i \in \Iset_i$ define $\pi^\sigma(I_i) = \sum_{h \in I_i}\pi^\sigma(h)$, as the probability of reaching information set $I_i$ given all players play according to $\sigma$. $\pi_i^\sigma(I_i)$ and $\pi_{-i}^\sigma(I_i)$ are defined similarly. Finally, let $\pi^\sigma(h,z) = \frac{\pi^\sigma(z)}{\pi^\sigma(h)}$ if $h \sqsubset z$, and zero otherwise. $\pi^\sigma_i(h,z)$ and $\pi^\sigma_{-i}(h,z)$ are defined similarly. Using this notation, \textit{expected payoff} for player $i$ is $u_i(\sigma) = \sum_{z \in Z}u_i(z)\pi^\sigma(z)$. A \textit{best response} (BR) of player $i$ to the opponent's strategy $\sigma_{-i}$ is a strategy $\sigma_i^{BR} \in BR_i(\sigma_{-i})$, where $u_i(\sigma_i^{BR}, \sigma_{-i}) \geq u_i(\sigma'_i, \sigma_{-i})$ for all $\sigma'_i \in \Sigma_i$. A tuple of strategies $( \sigma_i^{NE}, \sigma_{-i}^{NE})$, $\sigma_{i}^{NE}\in\Sigma_{i}, \sigma_{-i}^{NE}\in\Sigma_{-i}$ is a \emph{Nash Equilibrium} (NE) if $\sigma_i^{NE}$ is an optimal strategy of player $i$ against strategy $\sigma_{-i}^{NE}$. Formally: $\sigma_i^{NE} \in BR(\sigma_{-i}^{NE})\quad\forall i\in \{\pr,\ps \}$.

In a two-player zero-sum game, the \textbf{exploitability} of a strategy is defined as the expected utility a fully rational opponent can achieve above the value of the game. Formally, exploitability $\mathcal{E}(\sigma_i)$ of strategy $\sigma_i\in\Sigma_i$ is
$
    \mathcal{E}(\sigma_i) =  u_{-i}(\sigma_i, \sigma_{-i}) - u_{-i}(\sigma^{NE}), \quad \sigma_{-i} \in BR_{-i}(\sigma_i).
$

We define \textbf{gain} of a strategy against a sub-rational opponent as an expected utility we receive above the value of the game. Formally, gain $\mathcal{G}(\sigma_i, \sigma_{-i})$ of strategy $\sigma_i$ against strategy $\sigma_{-i}$ is defined as
$
\mathcal{G}(\sigma_i, \sigma_{-i}) = u_i(\sigma_i, \sigma_{-i}) - u_{i}(\sigma^{NE}).
$



\paragraph{Depth-limited Solving}
We denote $H_i(h)$ the sequence of player $i$'s information states and actions on the path to a history $h$. Two histories $h, h'$ where player $i$ does not act are in the same \textit{augmented information set} $I_i$ if $H_i(h) = H_i(h')$. We partition the game histories into \textbf{public states} $PS_i \subset H$, which are closed under the membership within the augmented information sets of all players. \textbf{Trunk} is a set of histories $T \subset H$, closed under prefixes and public states. \textbf{Subgame} $S \subset H$ is a forest of trees closed under extensions and public states. \textbf{Range} of a player $i$ is a probability distribution over his information sets in some public state $PS_i$, given we reached the $PS_i$. \textbf{Value function} is a function that takes the public state and both players' ranges as input and outputs values for each information set in the public state for both players. We assume using an approximation of an \textbf{optimal value function}, which is a value function returning the values of using some NE after the depth-limit. \textbf{Subgame partitioning} $\mathcal{P}$ is a partitioning that splits the game into trunk and subgames into multiple different levels based on some depth-limit or other factors (domain knowledge). Subgame partitioning can be naturally created using the formalism of factored-observation stochastic games. \cite{kovavrik2019value}. We denote by $u_i(\sigma)^T_V$ the utility for player $i$ if we use strategy profile $\sigma$ in trunk $T$ and compute values at the depth-limit using value function $V$.

% \subsection{Gadgets}
% When resolving a subgame we can add a chance node at the beginning that will aggregate the probabilities of all the players that the root states are reached. However, there is no guarantee on the resulting exploitability of the strategy in the full game and the exploitability can raise significantly \cite{burch2014solving}. To address the issue \textit{gadgets} are used to limit the increase in exploitability.

% \paragraph{Resolving Gadget}
% The resolving gadget \cite{burch2014solving} is the gadget that creates an initial chance node by aggregating only reaches of chance and the resolving player. The chance node can be normalized, and we would then multiply terminals by the normalization factor, which is equivalent. Instead of the opponent's strategy, it adds a node after each initial chance action, where the opponent can follow and play the game as it is normally played or terminate. In that case, it will receive the counterfactual best response value in that information set, saved from the previous step. 

% \paragraph{Max-margin Gadget}
% The gadget used to improve the resolved strategy is the max-margin gadget \cite{moravcik2016refining}. It starts with a node for player $\ps$, which allows him to choose his beliefs freely. Then after each action from the initial node, the chance node follows, which assigns probabilities to nodes in the chosen information set using the aggregated reaches of both chance and resolving players.

==> old_sections/03_suggested_approaches.tex <==
\section{Continual Depth-limited Responses}
\label{sec:concepts}
This section formally defines the strategies we are computing and the practical algorithms we use. The pseudo-code of the algorithms is in Algorithm~\ref{alg:cdbr}.

\subsection{Using Only the Optimal Value Function}
When we add the opponent model to the depth-limited solving, the exact solution would require capturing the opponent's mistakes after the depth-limit given by the opponent model in the value function. Training the value function is costly. Hence, it is infeasible for many opponent models and outright impossible for applications where we do not know the model in advance and gradually update it after each interaction. We instead explore the effects of using \textbf{only the optimal value function}. We start from the top of the game and construct a trunk with a depth-limit. Next, we solve the trunk, using the value function to evaluate public states at the depth-limit. Then we move forward to the next public state reached in the game, and we construct a subgame starting from the public state with some depth-limit. We solve the depth-limited subgame and continue with the same steps until we reach the end of the game.

The main problem of depth-limited solving is that when we find the equilibrium in the subgame, the joined strategy from trunk and subgame together is not guaranteed to be Nash equilibrium and can be substantially exploitable. To solve the issue, we can use \textbf{gadget} \cite{burch2014solving, moravcik2016refining, brown2017safe}, which adds a structure above the root of the subgame and using the summary values from previous iterations guarantees the exploitability will not rise.

\begin{figure}
    \centering
    \vspace{-5mm}
    \includegraphics[width=\linewidth]{graphics/christmas_tree.pdf}
    \caption{Illustration of the depth-limited solving.}
    \label{fig:subgames}
    \vspace{-2mm}
\end{figure}

\subsection{Continual Depth-limited Best Response}
Given any extensive-form game $G$ with perfect recall, opponent's fixed strategy $\sigma_\ps^F$ and some subgame partitioning $\partition$, we define continual depth-limited best response (CDBR) recursively from the top, see Figure~\ref{fig:subgames}. First we have trunk $T_1 = T$ and value function $V$. CDBR in the trunk $T_1$ for player $\pr$ with value function $V$ is defined as $\sbr(\sigma_\ps^F)_V^{T_1} = \argmax_{\sigma_\pr}u_\pr(\sigma_\pr, \sigma_\ps^F)_V^{T_1}$. In other words, we maximize the utility over the strategy in the trunk, where we return values from the value function after the depth-limit. In each step afterwards we create a new subgame $S_i$ and create new trunk by joining the old one with the subgame, creating $T_i = T_{i-1} \cup S_i$. We fix the strategy of player $\pr$ in the $T_{i-1}$ and maximize over strategy in the subgame. $\sbr(\sigma_\ps^F)_V^{T_i} = \argmax_{\sigma_\pr^{S_i}}u_\pr(\sigma_\pr^{S_i} \cup \sigma_\pr^{T_{i-1}}, \sigma_\ps^F)_V^{T_i}$. We continue like that for each step, and we always create a new trunk $T_i$ using the strategy from step $T_{i-1}$ until we reach the end of the game. We denote the full CDBR strategy created by joining strategies from all possible branches $\sbr(\sigma_\ps^F)_V^\mathcal{P}$.

\subsubsection{Computing CDBR}
The algorithm's input is the game's definition and the opponent's strategy. We have a fixed solving depth, such that the created subgames can fit in the memory, and we can solve them in a reasonable time. First, we get the trunk from the subgame partitioning. We need to compute the best response in the trunk given the value function, and since the output of the value function changes when strategy in the trunk changes, we can no longer compute the best response in one pass as in a full game. We need to use some version of CFR \cite{tammelin2015solving, brown2019solving, farina2020faster} and construct the strategy iteratively. Lemma~\ref{lem:convergence} in Section~\ref{sec:theory} shows that it converges to the best response in the trunk even if we only keep strategy from the best iteration without the need to compute the average strategy as in regular use of CFR.

After we solve the trunk, we move into the subgame, and we use value resolving without any gadgets because the opponent can not change his strategy in the trunk. We set the initial reaches in the subgame using player strategies and chance. We then solve the resulting subgame using depth-limited CFR.

\subsection{Continual Depth-limited RNR}
Given any extensive-form game $G$ with perfect recall, restricted Nash response can be computed by solving a modified game \cite{johanson2008computing}: We add an initial chance node with two outcomes that player $\pr$ does not observe. We copy the whole game $G$ after both outcomes of the chance node. In one tree, the opponent plays the fixed strategy, and we denote it $G^F$. The other tree is the same as the original game; we mark it $G'$. Player $\pr$ does not observe the initial chance node his infosets span over both $G'$ and $G^F$. We denote the full modified game $G^M$. Parameter $p$ is the initial chance node probability of picking $G^F$. Given the opponent's fixed strategy $\sigma_\ps^F$ and some subgame partitioning $\mathcal{P}$ of $G^M$ we define continual depth-limited restricted Nash response (CDRNR) recursively from the top. First we have trunk $T_1^M$ using $\mathcal{P}$ and value function $V$. Note that the number and semantic of infosets at the value function for player $\pr$ remain unchanged, and for $\ps$, inputs and outputs are doubled in size, so the value function is a bit more complex. CDRNR for player $\pr$ in the trunk $T_1^M$ using value function $V$ is $\srnr(\sigma_\ps^F, p)_V^{T_1^M} = \argmax_{\sigma_\pr}u_\pr(\sigma_\pr, BR(\sigma_\pr))_V^{T_1^M}$. And then in every following step we create the new subgame $S_i^M$ and enlarge the trunk to incorporate this subgame, creating trunk $T_i^M$ = $T_{i-1}^M \cup S_i^M$. Next, we fix strategy $\sigma_\pr^{T_{i-1}^M}$ of player $\pr$ in the previous trunk $T_{i-1}^M$ so it can not be changed anymore and the CDRNR is $\srnr(\sigma_\ps^F, p)_V^{T_i} = \argmax_{\sigma_\pr^{S_i^M}} u_\pr(\sigma_\pr', BR(\sigma_\pr'))_V^{T_i^M}$ where $\sigma_\pr'$ is a combination of the strategy we optimize over and the fixed strategy from previous step, formally $\sigma_\pr' = \sigma_\pr^{S_i^M} \cup \sigma_\pr^{T_{i-1}^M}$.

To summarize, we optimize only over the strategy in the subgame used in the current step while the strategy in the previous parts of the game is fixed for player $\pr$, and we give the opponent a chance to best respond in the whole $T'_i$. We denote the full CDRNR strategy $\srnr(\sigma_\ps^F, p)_V^\partition$.

\subsubsection{Computing CDRNR}
The input for computing CDRNR is also a definition of the game, opponent strategy, value function with the same inputs and outputs as CDBR, and the parameter $p$. We can create a modified game $G^M$ explicitly, or we can use the original game tree and store everything in it because the trees are identical. The trunk is solved using depth-limited CFR with the value function, where both players act, but the opponent changes his strategy only in $G'$. We play following the strategy in the trunk, and when we need to play outside of the trunk, we need to create a new depth-limited game.

We create a new depth-limited game in the same way as we specify in the concept. Unlike CDBR, we can not exchange the trunk for the chance node because player $\ps$ can deviate in the $G'$ part. We then need to use the value function when leaving the trunk. This means that we can not exchange the trunk part of $G^F$ because the value function still needs the reach probabilities from the fixed part of the tree. However, we can compute the reaches once and reuse them because we know they will not change and do not need the returned values. To summarize, we construct the new depth-limited game by appending the new subgame to the trunk.

Then we resolve the subgame by CFR with value function, and we play according to the resolved strategy in the subgame. When we leave the subgame, we construct a new subgame and continue until the game ends.

The approach is computationally more demanding than CDBR, but it only grows polynomially with each resolving round making it tractable. We attempted to exchange the trunk using existing gadgets \cite{burch2014solving, moravcik2016refining, brown2017safe}, and we found out all the existing gadgets work nicely for standard resolving but break when we insert the model.

\begin{algorithm}
\caption{Computing CDBR (CDRNR)}\label{alg:cdbr}
\begin{algorithmic}
\Require game $G$, opponent strategy $\sigma_\ps^F$, value function $V$
\State create (virtually) modified game $G^M$ (only CDRNR)
\State create subgame partitioning $\partition$ from $G$ ($G^M$)
\State $\sigma_\pr^\sbr$ = empty strategy ready to be filled
\State $I$ = initial information set in which we act
\State $S$ = $\empty$ current constructed subgame
\While{$I$ not null}
\If{$I$ not in $S$}
    \State S = construct new $S$ from $\partition$ using previous $S$ (CDRNR does not delete trunk)
    \State $\sigma_\pr^\sbr$ += solution of $S$ using CFR+ with $V$
\Else
    \State pick action $A$ according to $\sigma_\pr^\sbr$ in $I$
    \State get new $I$ using $A$ (or null if the game ends)
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

==> old_sections/04_gadgets.tex <==
\section{Why Gadgets Fail}
\label{sec:gadgets}
To demonstrate the problem with using gadgets, it is sufficient to assume that the subgame is constructed until the end of the game without using value functions. The problem shows when we solve the game from a non-root public state.
In RNR, the chance node at the beginning is not observed by player $\pr$. Therefore, in each information set, player $\pr$ chooses his actions based on the values of his actions combined from the values in $G'$ and $G^F$.
The values in $G^F$ can be computed without problem even if we do not start from the beginning since the opponent's strategy is fixed.
However, in $G'$ player $\ps$ can respond, and we need to make sure the values of the part of the information set in $G'$ are also \emph{correct}. Formally:

\begin{definition}
    For each information set $I \in \Iset_{\pr}$ we need the value of it's part in $G'$, formally $\sum_{h \in I, h \in G', z \in Z, h \sqsubset z}\pi^\sigma(z)u_{\pr}(z)$, to be the same as the value we would get if we let player $\ps$ play BR in full $G'$.
    \label{def:value}
\end{definition}

We can then apply the value function, and the problem will still be the same because it is related to the history we are forgetting while the value function is applied looking forward in the game. In the following examples, we show the requirement is not satisfied for common resolving gadgets. We tried to construct a gadget which would satisfy the condition, but in the end, we kept the previously resolved parts of the game $G'$ which satisfies the condition, and still only increased the size of the solved part of the game linearly. The construction of a constant-size gadget fulfilling the previous condition is an open problem.

\subsection{Restricted Nash Response with Gadget}
 We show that commonly used resolving gadgets are either overestimating or underestimating the values from Definiton~\ref{def:value} on an example game in Figure~\ref{fig:gadget_problem_resolving_gadget}. In the game, we first randomly pick a red or green coin. Player $\ps$ observes this and decides to place the coin heads up (RH, GH) or tails up (RT, GT). Player $\pr$ can not observe anything and, in the end, chooses whether he wants to play the game (P) or quit (Q).

In equilibrium, player $\pr$ plays action $Q$, and player $\ps$ can mix action up to the point where utility for $P$ is at most 0. This gives the value of the game 0, and counterfactual values in all inner nodes are also 0. If we assume the modified RNR game $G^M$ with an opponent model that makes it worth for player $\pr$ to play (P) in the game, $\ps$ will play $(RH,GH)$ in $G'$ with utility -3 for player $\pr$ in $G'$. We will use gadgets to resolve the game beginning in the player $\pr$ information set.

\def\istgamescale{0.8}
\begin{figure*}
    \begin{minipage}{0.32\linewidth}
        \centering
        \scalebox{1.012}{
            \begin{istgame}
            \setistOvalNodeStyle{.5cm}
            \setistRectangleNodeStyle{.5cm}
            \xtShowTerminalNodes[rectangle node]
            \istrooto(0){c}+{4.5mm}..{2.4cm}+
                \istb{0.5}[left, xshift=4mm, yshift=2.2mm]  \istb{0.5}[right, xshift=-4mm, yshift=2.2mm]  \endist
            \istrooto(1)(0-1){$\ps$}+{8.5mm}..{1.2cm}+
                \istb{RH}[left, xshift=1.5mm, yshift=2mm]  \istb{RT}[right, xshift=-1.5mm, yshift=2mm]  \endist
            \istrooto(2)(0-2){$\ps$}+{8.5mm}..{1.2cm}+
                \istb{GH}[left, xshift=1.5mm, yshift=2mm]  \istb{GT}[right, xshift=-1.5mm, yshift=2mm]  \endist
            \istrooto(3)(1-1){$\pr$}+{8.5mm}..{.6cm}+
                \istbt{P}[l]{-4}[center]  \istbt{Q}[r]{0}[center]  \endist
            \istrooto(4)(1-2){$\pr$}+{8.5mm}..{.6cm}+
                \istbt{P}[l]{-1}[center]  \istbt{Q}[r]{0}[center]  \endist
            \istrooto(5)(2-1){$\pr$}+{8.5mm}..{.6cm}+
                \istbt{P}[l]{-2}[center]  \istbt{Q}[r]{0}[center]  \endist
            \istrooto(6)(2-2){$\pr$}+{8.5mm}..{.6cm}+
                \istbt{P}[l]{10}[center]  \istbt{Q}[r]{0}[center]  \endist
            \xtInfoset(1-1)(1-2)
            \xtInfoset(1-2)(2-1)
            \xtInfoset(2-1)(2-2)
            \end{istgame}
        }
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \scalebox{\istgamescale}{
            \begin{istgame}
            \setistOvalNodeStyle{.5cm}
            \setistRectangleNodeStyle{.5cm}
            \xtShowTerminalNodes[rectangle node]
            \istrooto(0){c}+{10.5mm}..{1.8cm}+
                \istb{0.5}[left, xshift=0mm, yshift=0.5mm]  \istb{0.5}[left, xshift=1mm, yshift=0.5mm] \istb{0.5}[right, xshift=-1mm, yshift=0.5mm] \istb{0.5}[right, xshift=0mm, yshift=0.5mm]  \endist
            \istrooto(1)(0-1){$\ps$}+{8.5mm}..{0.9cm}+
                \istb{F}[left, xshift=1.5mm, yshift=2mm]  \istbAt<level distance=1.2*\xtlevdist>{T}[right, xshift=-0.8mm, yshift=2.8mm]{0}[center]  \endist
            \istrooto(2)(0-2){$\ps$}+{8.5mm}..{0.9cm}+
                \istb{F}[left, xshift=1.5mm, yshift=2mm]  \istbAt<level distance=1.2*\xtlevdist>{T}[right, xshift=-0.8mm, yshift=2.8mm]{0}[center]  \endist
            \istrooto(3)(0-3){$\ps$}+{8.5mm}..{0.9cm}+
                \istb{F}[left, xshift=1.5mm, yshift=2mm]  \istbAt<level distance=1.2*\xtlevdist>{T}[right, xshift=-0.8mm, yshift=2.8mm]{0}[center]  \endist
            \istrooto(4)(0-4){$\ps$}+{8.5mm}..{0.9cm}+
                \istb{F}[left, xshift=1.5mm, yshift=2mm]  \istbAt<level distance=1.2*\xtlevdist>{T}[right, xshift=-0.8mm, yshift=2.8mm]{0}[center]  \endist
            \istrooto(5)(1-1){$\pr$}+{9.5mm}..{.6cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{-4}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \istrooto(6)(2-1){$\pr$}+{9.5mm}..{.6cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{-1}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \istrooto(7)(3-1){$\pr$}+{9.5mm}..{.6cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{-2}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \istrooto(8)(4-1){$\pr$}+{9.5mm}..{.6cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{10}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \xtInfoset(1-1)(2-1)
            \xtInfoset(2-1)(3-1)
            \xtInfoset(3-1)(4-1)
            \end{istgame}
        }
    \end{minipage}
    \begin{minipage}{0.32\linewidth}
        \centering
        \scalebox{\istgamescale}{
            \begin{istgame}
            \setistOvalNodeStyle{.5cm}
            \setistRectangleNodeStyle{.5cm}
            \xtShowTerminalNodes[rectangle node]
            \istrooto(0){$\ps$}+{10.5mm}..{1.6cm}+
                \istb{E}[left, xshift=0mm, yshift=0.8mm]  \istb{F}[left, xshift=1mm, yshift=0.5mm] \istb{G}[right, xshift=-1mm, yshift=0.5mm] \istb{H}[right, xshift=0mm, yshift=0.8mm]  \endist
            \istrooto(1)(0-1){c}+{8.5mm}..{0.8cm}+
                \istb{0.5}[left, xshift=0mm, yshift=1mm] \endist
            \istrooto(2)(0-2){c}+{8.5mm}..{0.8cm}+
                \istb{0.5}[left, xshift=0mm, yshift=1mm] \endist
            \istrooto(3)(0-3){c}+{8.5mm}..{0.8cm}+
                \istb{0.5}[left, xshift=0mm, yshift=1mm] \endist
            \istrooto(4)(0-4){c}+{8.5mm}..{0.8cm}+
                \istb{0.5}[left, xshift=0mm, yshift=1mm] \endist
            \istrooto(5)(1-1){$\pr$}+{9.5mm}..{.8cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{-4}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \istrooto(6)(2-1){$\pr$}+{9.5mm}..{.8cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{-1}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \istrooto(7)(3-1){$\pr$}+{9.5mm}..{.8cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{-2}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \istrooto(8)(4-1){$\pr$}+{9.5mm}..{.8cm}+
                \istbt{P}[left, yshift=-0.5mm, xshift=0.5mm]{10}[center]  \istbt{Q}[right, yshift=-0.5mm, xshift=-0.5mm]{0}[center]  \endist
            \xtInfoset(8)(7)
            \xtInfoset(7)(6)
            \xtInfoset(6)(5)
            \end{istgame}
        }
    \end{minipage}
    \caption{(left) Game to show problems with gadgets. (middle) Resolving gadget for the left game. (right) Max-margin and Reach max-margin gadget.}
    \label{fig:gadget_problem_resolving_gadget}
\end{figure*}
\paragraph{Resolving Gadget} \cite{burch2014solving}
Resolving gadget on the game in Figure~\ref{fig:gadget_problem_resolving_gadget} has all utilities after \textit{terminate} actions 0. When we resolve the gadget, the utility is 0. However, when player $\pr$ deviates to action $P$, player $\ps$ plays \textit{follow} action in all but the rightmost node, and the utility of player $\pr$ will be -3.5. Therefore, the common resolving gadget may overestimate the real exploitability of the strategy in the subgame. Overestimating may lead to not exploiting as much as we can and makes it impossible to prove Theorem~\ref{thm:SRNR nash} about the minimal gain of our algorithm. It might seem that normalization of the chance node could solve the problem, but it would only halve the value to -1.75, which is still incorrect.

\paragraph{(Reach) Max-margin Gadget} \cite{moravcik2016refining, brown2017safe}
All the counterfactual best response values are 0, and we do not need to offset any node in the max-margin gadget. Similarly, the reach max-margin gadget offsets the values using counterfactual values. It adds a lower bound on previous mistakes, but since we assume both players played perfectly before the depth limit, the offset is also 0. Then both gadget constructions are identical. We add the initial decision node and the chance nodes (since there is only one state in each infoset, the nodes have only one action). When we solve the gadget, player $\pr$ will pick action $Q$, and the gadget value will be 0. However, when player $\pr$ deviates to action $P$, player $\ps$ now has a choice between terminal utilities and picks action $E$ to receive the highest one. This will result in utility -2, and we see that (reach) max-margin gadgets can underestimate the real exploitability. Underestimating the exploitability can lead to our algorithm being more exploitable than we want using some $p$, and it makes Theorem~\ref{thm:DBR nash} impossible to prove. Similar to the previous gadget, normalizing the chance nodes would lead to double the utility, which is still incorrect.

\paragraph{Full Gadget vs Other Gadgets}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{graphics/gadget_breaking.pdf}    
    \caption{Comparison of Gain and Exploitability of the solutions using Full gadget compared to other gadgets.}
    \label{fig:g_break}
\end{figure}

We show that other gadgets can overestimate or underestimate exploitability, which could simply shift the distribution of the parameter $p$ and we could still compute the same solutions. However, in Figure~\ref{fig:g_break} we show the results on a game created to break the other gadgets. The game has five actions for the exploiter and each one is crucial in reconstructing the full RNR set. Full gadget is able to recover all five actions using different $p$ but other gadgets can only compute two actions regardless of the choice of $p$.

==> old_sections/05_theory.tex <==
\section{Theory}
\label{sec:theory}
This section provides the theoretical performance guarantees for CDBR and CDRNR and explains why the guarantee can not be even better. Furthermore, we provide an upper bound on the exploitability of CDRNR, linking it to the gain by the parameter $p$. Formal proofs of all the theorems are in the appendix.

\subsection{Response Performance Against Model}
The first theorem shows that CDBR and CDRNR will achieve at least the value of the game against the opponent model. Theorem specifically for CDBR is only in the appendix because it is only a special case of Theorem~\ref{thm:SRNR nash}. However, as shown in the appendix, CDBR can perform worse than a Nash equilibrium against the fixed opponent because of the perfect opponent assumption at the depth-limit.

\begin{lemma}
Let $G$ be a zero-sum imperfect-information extensive-form game with perfect recall. Let $\sigma_\ps^\text{F}$ be fixed opponent's strategy, and let $T$ be some trunk of the game. If we perform CFR iterations in the trunk for player $\pr$ then for the strategy $\hat{\sigma}_{\pr}$ from the iteration with highest expected utility it holds $\max_{\sigma_{\pr}^* \in \Sigma_\pr} u_\pr(\sigma_{\pr}^*, \sigma_\ps^F)_V^T - u_\pr(\hat{\sigma}_{\pr}, \sigma_\ps^F)_V^T \leq \Delta\sqrt{\frac{A}{T}}|\mathcal{I}_{TR}| + TN_S\epsilon_S$ where $\Delta$ is variance in leaf utility, $A$ is an upper bound on the number of actions, $|\mathcal{I}_{TR}|$ is number of information sets in the trunk, $N_S$ is the number of information sets at the root of any subgame and value function error is at most $\epsilon_S$.
\label{lem:convergence}
\end{lemma}

The previous lemma states that the algorithm in CDBR converges to the best response in the trunk not only using an average strategy which is guaranteed by CFR but also if we track the strategy with the highest utility, it will converge to the best response.

For the following theorems, we denote $\mathcal{S}$ as the set consisting of the trunk and all the subgames explored when computing the response, and $\mathcal{S'}$ is the same but without the last subgame. $S^B$ denotes a border of the subgame (a set of all the states where the value function is used in the subgame). We also denote $S^O$ the set of all the states where we leave the trunk not going in the currently resolving subgame (set of the states where value function is used in RNR which are not in $S^B$).

\begin{theorem}
Let $G$ be any zero-sum extensive-form game with perfect recall and let $\sigma_\ps^\text{F}$ be any fixed opponent's strategy in $G$. Then we set $G^M$ as restricted Nash response modification of $G$ using $\sigma_\ps^\text{F}$. Let $\mathcal{P}$ be any subgame partitioning of the game $G^M$ and using some $p \in \langle0,1\rangle$, let $\sigma_\pr^{\srnr}$ be a CDRNR given approximation $\bar{V}$ of the optimal value function $V$ with error at most $\epsilon_V$ and opponent strategy $\sigma_\ps^\text{F}$ approximated in each step with regret at most $\epsilon_R$, formally $\sigma_\pr^{\srnr} = \srnr(\sigma_\ps^F, p)_V^\mathcal{P}$. Let $\sigma^{NE}$ be any Nash equilibrium in $G$. Then $u_\pr(\sigma_\pr^{\srnr}, \sigma_\ps^F) + \sum_{S \in \mathcal{S'}}|I_{S^O}|(1-p)\epsilon_V + |\mathcal{S}|\epsilon_R + \sum_{S \in \mathcal{S'}}|I_{S^B}|\epsilon_V \geq u_\pr(\sigma^{NE})$.
\label{thm:SRNR nash}
\end{theorem}

The previous theorem states that our approaches have the first property we wanted, and when we respond to the model, we will receive at least the value of the game.

\subsection{Exploitability Guarantee of CDRNR}
\begin{theorem}
Let $G$ be any zero-sum extensive-form game with perfect recall and let $\sigma_\ps^\text{F}$ be any fixed opponent's strategy in $G$. Then we set $G^M$ as restricted Nash response modification of $G$ using $\sigma_\ps^\text{F}$. Let $\mathcal{P}$ be any subgame partitioning of the game $G^M$ and using some $p \in \langle0,1\rangle$, let $\sigma_\pr^{\srnr}$ be a CDRNR given approximation $\bar{V}$ of the optimal value function $V$ with error at most $\epsilon_V$, partitioning $\mathcal{P}$ and opponent strategy $\sigma_\ps^\text{F}$, which is approximated in each step with regret at most $\epsilon_R$, formally $\sigma_\pr^{\srnr} = \sigma_\pr^\srnr(\sigma_\ps^F, p)_V^\mathcal{P}$. Then exploitability has a bound $\mathcal{E}(\sigma_\pr^\srnr) \leq \mathcal{G}(\sigma_\pr^\srnr, \sigma_\ps^F)\frac{p}{1-p} \sum_{S \in \mathcal{S'}}|I_{S^O}|(1-p)\epsilon_V + |\mathcal{S}|\epsilon_R + \sum_{S \in \mathcal{S'}}|I_{S^B}|\epsilon_V$, $\mathcal{E}$ and $\mathcal{G}$ are defined in Section~\ref{sec:background}.
\label{thm:DBR nash}
\end{theorem}

The last theorem is more complex, and it bounds the exploitability by the gain of the strategy against the model. With $p = 0$ it is reduced to the continual resolving and with $p = 1$ to CDBR with unbounded exploitability. The theorem shows we can manipulate allowed exploitability by changing the $p$.

==> old_sections/06_experiments.tex <==
\section{Experiments}
We show a comparison between continual depth-limited best response (CDBR) and local best response (LBR) \cite{lisy2017eqilibrium}. We also show empirically that the continual depth-limited restricted Nash response (CDRNR) exploitability is bounded, and we explore the tradeoff between exploitability and gain in CDRNR. The appendix contains hardware setup, domain description, algorithm details, and experiments on more game domains. We use two types of opponent strategies, strategies generated by a low amount of CFR iterations and random strategies with different seeds.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{graphics/cdrnr_leduc_01.pdf}
    \includegraphics[width=1\linewidth]{graphics/cdrnr_leduc_0.5.pdf}
    \caption{Gain and exploitability comparison of BR, RNR, CDRNR, SES and best Nash equilibrium (BNE) in Leduc Hold'em (top) against strategies from CFR using a small number of iterations with different $p$ values. The \textbf{a} stands for the average of the other values. VF is CDRNR using an imperfect value function. SX is CDRNR with perfect value function using lookahead with X steps.}
    \label{fig:expl}
\end{figure}

\subsection{Exploitability of Robust Responses}
We report both gain and exploitability for CDRNR on Leduc Hold'em. Results in Figure~\ref{fig:expl} show that the proven bound on exploitability works in practice, and we see that the bound is very loose in practice. For example, with $p=0.5$, the bound on the exploitability is the gain itself, but the algorithm rarely reaches even a tenth of the gain in exploitability. This shows that the CDRNR is similar to the restricted Nash response because, with a well-set $p$, it can significantly exploit the opponent without significantly raising its exploitability. The only exception is the CDRNR with value function, which shows the added constants from the value function's imprecision. When the opponent is close to optimal, we see that the exploitability can rise above the gain.

In most cases, the gain and exploitability of CDRNR are lower than that of RNR. Gain must be lower because of the different value function, but the exploitability can be higher, as seen with $p=0.1$ against low iteration strategies. The depth-limited scheme causes that, and because the algorithm, unlike RNR, has not complete information when making individual decisions, it can choose different paths to exploit the opponent, raising its exploitability more than it has to. However, the bound will always hold. We provide results on other domains and for more parameter values $p$ in the appendix.

We also compare the algorithm against the best possible Nash equilibrium. It is computed by a linear program and serves as the theoretical limit of maximal gain, which does not allow exploitability. It would be impossible to compute for larger games. We can see we can gain twice as much with exploitability still being almost zero.

We report the result with the value function produced by 500 CFR iterations as VF. We split the Leduc by rounds, so it does not correspond to any step scheme and is somewhere between S1 and S5. As expected, the imperfect value function slightly decreases the performance, but overall is comparable to the algorithms using the optimal value function.

Last comparison is with SES, which performs poorly and is only slightly above the best Nash equilibrium in terms of Gain. On the other hand it is almost not exploitable.

\subsection{Local Best Response vs. CDRNR}
We compare LBR and CDBR in Leduc Holde'm. We also compare CDBR with just the BR in imperfect information Goofspiel, but without LBR, which is poker specific. We show that CDBR and LBR are very similar with smaller steps, and as we increase the depth-limit of CDBR, it starts outperforming LBR. The behavior differs in every strategy because LBR assumes the player continues the game by only calling till the end, while CDBR uses the perfectly rational extension. Furthermore, it is possible to exchange the value function of CDBR, and both concepts would be very similar. However, we would lose the guarantee that CDBR will never perform worse than the value of the game.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{graphics/lbr_sbr.pdf}
    \includegraphics[width=1\linewidth]{graphics/gain_iigs5.pdf}
    \caption{Gain comparison of best response (BR), local best response (LBR - only poker), and continual depth-limited best response (CDBR) in Leduc Hold'em (top) and Imperfect information Goofspiel (bottom) against strategies from CFR using a small number of iterations (left) and random strategies (right). The \textbf{a} stands for the average of the other values in the plot. The number after CDBR stands for the number of actions CDBR was allowed to look in the future, and CDBRNN is one step CDBR with a neural network as a value function.}
    \label{fig:lbrsbr}
\end{figure}

Looking at the results in Figure~\ref{fig:lbrsbr}, we can see that both concepts are good at approximating the best response, with CDBR being better against both strategies. LBR looks at one following action, so in terms of comparability, it is best compared to the CDBR1. Next, we observe a lack of monotonicity in step increase, which is linked to the counterexample in the appendix. When we increase the depth-limit, the algorithm can exploit some early mistake that causes it to miss a sub-tree where the opponent makes a much bigger mistake in the future. Finally, we can see the difference between the algorithm with guarantees and LBR without them nicely. Against strategy from 34 CFR iterations, LBR can no longer achieve positive gain and only worsens with more iterations. In contrast, CDBR can always achieve at least zero gain (assuming we have an optimal value function).

\subsection{Flop Hold'em}
The code does not work... I probably can not fix it in time
% Last experiment is on a Flop Hold'em, large game with 727 million infosets. We play first round using abstracted game, which leaves the trunk unabstracted but clusters possible board cards into only three options. After the board cards are dealt we resolve in an unabstracted game.

==> old_sections/07_related_work.tex <==
\section{Related Work}
This section describes the related work focusing more on distinguishing our novel contributions.

We have been inspired by the depth-limited solving used by DeepStack, and other algorithms \cite{moravvcik2017deepstack, brown2018superhuman}. Depth-limited solving is an approach that made solving huge imperfect-information games possible.

Restricted Nash response (RNR) \cite{johanson2008computing} is an opponent exploiting scheme. It solves the entire game and allows changing the trade-off between exploitability and gain. Essentially it always produces $\epsilon$ safe best response \cite{mccracken2004safe}.

However, it is impossible to compute RNR in huge games, and we fused the RNR approach with depth-limited solving creating a novel algorithm we call CDRNR. CDRNR is the first robust response calculation that can be done in huge games, enabling opponent modeling approaches in such games.

Local best response \cite{lisy2017eqilibrium} is an evaluation tool for poker. It uses given abstraction in its action space. It picks the best action in each decision set, looking at fold probability for the opponent in the next decision node and then assuming the game is called until the end. Our second algorithm CDBR is a generalization of the LBR because we can use it on any game solvable by depth-limited solving. We have explicitly defined value function, which we can exchange for different heuristics.

Approximate best response (ABR) \cite{timbers2020approximate} is also a generalization of the LBR and showed promising results in evaluating strategies. However, our approach focuses on opponent modeling, which requires crucial differences, such as quick re-computation against unseen models. ABR needs to independently learn the response for every combination of opponent and game, making it unusable in the opponent modeling scenario. Our algorithms learn a single domain-specific value function and can subsequently compute strategies against any opponent in the run-time. Furthermore, ABR and even our CDBR are extremely brittle, making it a bad choice if we are unsure about the opponent, which we often are at the start of a game against an unknown opponent. On the other hand, our second algorithm CDRNR tackles exactly this issue and provides powerful exploitation with very limited exploitability.

Safe exploitation search (SES) \cite{liu2022safe} is a similar method to the one we propose. However, there are two significant differences. First, the method uses max-margin gadget without the same analysis as we did. As a result the main theoretical result on safety is not correct and we provide counterexample in the appendix. Second, the method does not fix the opponent strategy at all and only uses opponent reaches, when resolving the subgame. As a result SES exploitation is extremely limited and as we show in experiments it is often worse than simply using best Nash equilibrium. On top of that there are games where it fundamentally can not exploit the opponent, notably any perfect information game with or without simultaneous moves.

==> old_sections/08_conclusion.tex <==
\section{Conclusion}
Opponent exploitation is an essential topic in computational game theory, and no previous approaches use continual resolving for opponent exploitation. We propose algorithms to quickly compute depth-limited best response and depth-limited restricted Nash response once we have the value function, creating the first robust response applicable to massive games. We prove the soundness of the methods in terms of gain against the opponents and safety against the worst-case adversary. Next, we show that common resolving gadgets can skew the subgame value. Finally, we empirically evaluate the algorithms on three different games. We show that we can achieve high exploitation with the optimal value function and outperform the domain-specific local best response on poker.

==> old_sections/09_counterexample.tex <==


\section{Counterexample}
\label{sec:gadgets}
This section describes an example game which needs all the actions of the opponent in order to resolve correctly in the RNR scenario.

\subsection{Properties}
RNR balances the gain and exploitability. It does so by expanding the player $\pr$'s infosets over both trees in the modified game. We can imagine it as if $\pr$ receives a mix of the reaches in $G'$ and $G^F$ in each of his infosets. $G'$ is attempting to fully exploit the $\pr$'s strategy while $\pr$ is exploiting the model fixed in the $G^F$. Thought the mix of the reaches the player then balances the gain and exploitability based on the parameter $p$. To make it possible we need to ensure the reaches in the $G'$ are correct, meaning the same as if we allowed $\ps$ to best respond in the whole $G'$. Our counterexample shows that removing any $\ps$'s node from the game or not using value function changes the reaches making the strategy more exploitable or less exploiting.

\subsection{Example Game}
The game is played in rounds. Figure~\ref{fig:example_break} shows an example with three rounds. Starting chance node has as many actions as rounds plus one. In each round player $\ps$ can choose to prepare for this round (p*) or continue (c*). $\pr$ can choose independently for each round to either stay (s*) or leave (l*). Staying gives some reward but leaving can give more, if the other player prepared. If player $\ps$ continues instead of preparing there is a chance node with two equally likely outcomes to either terminate the game or continue to the next round. Reward for staying is always 2 and reward for leaving in $n$th round is $2^{2n}$. In the last round, if player $\pr$ stayed the player $\ps$ can choose to make a mistake giving better payoff to player $\pr$. This payoff is $\frac{1}{4}$ of the payoff for leaving in this round given player $\ps$ prepared.

\subsection{All the Actions Are Necessary}
Player $\ps$ plays uniformly in the equilibrium and if we extend the game to create RNR he will always attempt to fix the mistakes made by changing G' so that the reach in both trees combined is the same as in the equilibrium. However, we can choose a strategy in $G^F$ which will make this balancing impossible and player $\ps$ will be unable to fix the play from some round forward. Our example picks a strategy which can be balanced but only barely. This will produce equilibrium for player $\pr$ and model with the strategy of $\ps$ will also combine to equilibrium. We solve depth-limited game until the point when $\pr$ plays. Then we add the subgame of the last round and we see that the opponent actually made a mistake. This is the small change that makes the strategy impossible but again only barely. Since it is delicately balanced removing only a single constraint from any previous round enables player $\ps$ to fix the strategy, which shows that every action is important for the correct reaches. 

Formally, if we set $p=0.5$, the strategy $\sigma$ of player $\ps$ in the $G'$ and his fixed strategy $\sigma^F$ need to fulfill an equation for each round $\sigma(ca)\times\cdots\times\sigma(cn) + \sigma^F(ca)\times\cdots\times\sigma^F(cn) = \frac{1}{2^{n-1}}$. We find a strategy which fulfills this for each round. What we need from the strategy is to not fulfill it for the last one when the $\ps$ makes a mistake. However we need it such that if we remove one of the equations it is actually possible to satisfy the last round constraint. (Removing of one constraint is equivalent to removing one node of player $\ps$ or exchanging value function in his play action for a fixed value.) This is possible for game of this structure with at least three rounds.

Working example for game in Figure~\ref{fig:example_break} is fixed strategy which continues in all rounds with probability $\frac{3}{5}$. In the $G'$ the player $\ps$ continues in round $a$ with probability $\frac{2}{5}$, in round $b$ with probability $\frac{7}{20}$ and in round $c$ with probability $\frac{57}{70}$. When we move to the next depth-limited game where $\ps$ makes the mistake it changes the dynamic and $\pr$ will want to stay in last round making $\ps$ always prepare changing the reaches and the strategy.

However, if we remove any subset of player $\ps$'s nodes, he can fix the strategy and player $\pr$ has different reaches in his nodes, and changes his strategy to one that does not exploit as well.

Full RNR version of the game from Figure~\ref{fig:example_break} and all the different cases with different nodes left out are described in the appendix along with the gadgets and strategy grafting \cite{waugh2009strategy}.

\begin{figure}
        \centering
            \begin{istgame}
            \setistOvalNodeStyle{.5cm}
            \setistRectangleNodeStyle{.5cm}
            \xtShowTerminalNodes[rectangle node]
            \istrooto(0){c}+{4.5mm}..{1.1cm}+
                \istbA<level distance=2*\xtlevdist>{\frac{1}{4}}[left, xshift=0mm, yshift=2mm]  
                \istb<missing>
                \istbA<level distance=0.87*\xtlevdist>{\frac{1}{4}}[right, xshift=-0.5mm, yshift=1.5mm]
                \istbA<level distance=3.13*\xtlevdist>{\frac{1}{4}}[right, xshift=-3mm, yshift=18.5mm]
                \istb<missing>
                \istb{\frac{1}{4}}[right, xshift=-2mm, yshift=4.2mm]
            \endist
            \istrooto(1)(0-1){$\pr$}+{8.5mm}..{0.8cm}+
                \istbt{sb}[left, xshift=0.8mm, yshift=0.8mm]{2}[center]
                \istbt{lb}[right, xshift=-0.8mm, yshift=1mm]{0}[center]
            \endist
            \istrooto(2)(0-3){$\pr$}+{8.5mm}..{0.8cm}+
                \istbt{sa}[left, xshift=1mm, yshift=0.8mm]{2}[center]  
                \istbt{la}[right, xshift=-1mm, yshift=1mm]{0}[center]
            \endist
            \istrooto(3)(0-6){$\ps$}+{8.5mm}..{2.4cm}+
                \istb{pa}[left, xshift=1.5mm, yshift=2mm]  
                \istb{ca}[right, xshift=-1.5mm, yshift=2mm]
            \endist
            \istrooto(4)(3-1){$\pr$}+{8.5mm}..{0.8cm}+
                \istbt{sa}[left, xshift=1mm, yshift=0.8mm]{0}[center]  
                \istbt{la}[right, xshift=-1mm, yshift=1mm]{4}[center]
            \endist
            \istrooto(5)(3-2){c}+{8.5mm}..{1.6cm}+
                \istb{0.5}[left, xshift=1.5mm, yshift=2mm]
                \istbt{0.5}[right, xshift=-0.8mm, yshift=1mm]{1}[center]
            \endist
            \istrooto(6)(5-1){$\ps$}+{8.5mm}..{2.2cm}+
                \istb{pb}[left, xshift=3.5mm, yshift=3mm]
                \istb{cb}[right, xshift=-2.8mm, yshift=3mm]
            \endist
            \istrooto(7)(6-1){$\pr$}+{8.5mm}..{0.8cm}+
                \istbt{sb}[left, xshift=0.5mm, yshift=1mm]{0}[center]  
                \istbt{lb}[right, xshift=-0.5mm, yshift=1mm]{16}[center]
            \endist
            \istrooto(8)(6-2){c}+{8.5mm}..{1cm}+
                \istb{0.5}[left, xshift=1.5mm, yshift=2mm]
                \istbt{0.5}[right, xshift=-0.5mm, yshift=1mm]{1}[center]
            \endist
            \istrooto(9)(8-1){$\ps$}+{8.5mm}..{1cm}+
                \istb{pc}[left, xshift=1.5mm, yshift=2mm]
                \istbt{cc}[right, xshift=-1mm, yshift=0.5mm]{1}[center]
            \endist
            \istrooto(10)(9-1){$\pr$}+{8.5mm}..{1cm}+
                \istb{sc}[left, xshift=0.5mm, yshift=0.5mm]
                \istbt{lc}[right, xshift=-0.5mm, yshift=0.5mm]{64}[center]
            \endist
            \istrooto(11)(0-4){c}+{8.5mm}..{1cm}+
                \istbt{sc}[left, xshift=0.5mm, yshift=0.5mm]{2}[center]
                \istbt{lc}[right, xshift=-0.5mm, yshift=0.5mm]{0}[center]
            \endist
            \istrooto(12)(10-1){$\ps$}+{8.5mm}..{1cm}+
                \istbt{c}[left, xshift=0.5mm, yshift=0.5mm]{16}[center]
                \istbt{m}[right, xshift=-0.5mm, yshift=0.5mm]{0}[center]
            \endist
            \xtInfoset(0-3)(3-1)
            \xtInfoset(0-1)(6-1)
            \xtInfoset(0-4)(9-1)
            \end{istgame}
    \caption{Example game which needs all the opponent actions when resolved.}
    \label{fig:example_break}
\end{figure}
